Control of growth of local heat release rate fluctuations to suppress thermoacoustic instability

This experimental study investigates the dynamical transition from stable operation to thermoacoustic instability in a turbulent bluff-body stabilized dump combustor. We conduct experiments to characterize the dynamical transition utilizing acoustic pressure and local heat release rate fluctuations. We observe the transition to thermoacoustic instability for these experiments as we decrease the equivalence ratio towards a fuel-lean setting. More importantly, we observe significant growth of local heat release rate fluctuations near the bluff-body well before the appearance of large-scale spatial or temporal patterns during the occurrence of thermoacoustic instability. By strategically positioning slots (perforations) on the bluff-body, we ensure the reduction of the growth of local heat release rate fluctuations at the stagnation zone near the bluff-body at operating conditions far away from the onset of thermoacoustic instability. This reduction in the local heat release rate fluctuations ensures that the transition to thermoacoustic instability is avoided. We find that modified configurations of the bluff-body that do not quench these local heat release rate fluctuations at the stagnation zone results in the transition to thermoacoustic instability. We also reveal that an effective suppression strategy based on the growth of local heat release rate fluctuations requires an optimization of the area ratio of the slots for a given bluff-body position. Further, the suppression strategy also depends on the spatial distribution of perforations on the bluff-body. Notably, an inappropriate distribution of the slots which does not quench the local heat release rate fluctuations at the stagnation zone may even result in a dramatic increase in amplitudes of pressure oscillations.

==> epstopdf.1 <==
.TH EPSTOPDF 1 "17 January 2014"
.\" $Id: epstopdf.1 32701 2014-01-17 18:09:54Z karl $
.SH NAME
epstopdf, repstopdf \- convert an EPS file to PDF
.SH SYNOPSIS
\fBepstopdf\fP [\fIoptions\fP] [\fIepsfile\fP]
.SH DESCRIPTION
By default, \fBepstopdf\fP converts the input PostScript file to PDF,
using Ghostscript.
.PP
\fBEpstopdf\fP transforms the Encapsulated PostScript file \fIepsfile\fP
(or standard input) so that it is guaranteed to start at the 0,0
coordinate, and it sets a page size exactly corresponding to the
BoundingBox.  Thus, the result needs no cropping, and the PDF MediaBox
is correct.  
.PP
PJL commands at the start of a file are removed.  DOS EPS binary files
(TN 5002) are supported.
.PP
If the bounding box in the input is incorrect, of course there will
be resulting problems.
.SH OPTIONS
Options may start with either "\fB-\fP" or "\fB--\fP", and may be
unambiguously abbreviated.  It is best to use the full option name in
scripts, though, to avoid possible collisions with new options in the
future.
.PP
General script options:
.IP "\fB--help\fP
display help message and exit
.IP "\fB--version\fP
display version information and exit
.IP "\fB--outfile\fP=\fIfile\fP"
write result to \fIfile\fP.  If this option is not given, and
\fB--nogs\fP or \fB--filter\fP is specified, write to standard output;
otherwise, the default is to construct the output file name by replacing
any extension in the input file with `.pdf'.
.IP "\fB--\fP[\fBno\fP]\fBdebug\fP"
write debugging info (default: off).
.IP "\fB--\fP[\fBno\fP]\fBexact\fP"
scan ExactBoundingBox (default: off).
.IP "\fB--\fP[\fBno\fP]\fBfilter\fP"
read standard input and (unless \fB--outfile\fP is given) write standard
output (default: off).
.IP "\fB--\fP[\fBno\fP]\fBgs\fP"
run Ghostscript (default: on).  With \fB--nogs\fP, output (to standard
output by default) the PostScript that would normally be converted; that
is, the input PostScript as modified by \fBepstopdf\fP.
.IP "\fB--\fP[\fBno\fP]\fBhires\fP"
scan HiresBoundingBox (default: off).
.IP "\fB--restricted\fP=\fIval\fP"
turn on restricted mode (default: [on for repstopdf, else off]);
this forbids the use of \fB--gscmd\fP and \fB--gsopt\fP and imposes
restrictions on the input and output file names according to the values
of openin_any and openout_any (see the Web2c manual, http://tug.org/web2c).
.PP
Options for Ghostscript (more info below):
.IP "\fB--gscmd\fP=\fIval\fP"
pipe output to \fIval\fP (default: [\fBgswin32c\fP on Windows, else \fBgs\fP])
.IP "\fB--gsopt\fP=\fIval\fP"
include \fIval\fP as one argument in the gs command (can be repeated),
.IP "\fB--gsopts\fP=\fIval\fP"
split \fIval\fP at whitespace, include each resulting word as an
argument in the gs command (can be repeated)
.IP "\fB--autorotate\fP=\fIval\fP"
set AutoRotatePages (default: None); recognized \fIval\fP choices:
None, All, PageByPage.  For EPS files, PageByPage is equivalent to All.
.IP "\fB--\fP[\fBno\fP]\fBcompress\fP"
use compression in the output (default: on).
.IP "\fB--device\fP=\fIdev\fP"
use -sDEVICE=\fIdev\fP (default: pdfwrite); not all devices are allowed
in restricted mode.
.IP "\fB--\fP[\fBno\fP]\fBembed\fP"
embed fonts (default: on).
.IP "\fB--pdfsettings\fP=\fIval\fP"
use -dPDFSETTINGS=/\fIval\fP (default is `prepress' if \fB--embed\fP,
else empty); recognized \fIval\fP choices: screen, ebook, printer,
prepress, default.
.IP "\fB--\fP[\fBno\fP]\fBquiet\fP"
use -q, a.k.a. -dQUIET (default: off).
.IP "\fB--res\fP=\fIdpi, dpi\fPx\fIdpi\fP"
set image resolution (default: [use gs default]); ignored if
\fB--debug\fP is set.
.IP "\fB--\fP[\fBno\fP]\fBsafer\fP"
use -d(NO)QUIET (default: true).
.PP
In addition to the specific options above, additional options to be used
with gs can be specified with either or both of the two cumulative
options \fB--gsopts\fP and \fB--gsopt.\fP
.PP
\fB--gsopts\fP takes a single string of options, which is split at
whitespace, each resulting word then added to the gs command line
individually.
.PP
\fB--gsopt\fP adds its argument as a single option to the gs command
line.  It can be used multiple times to specify options separately,
and is necessary if an option or its value contains whitespace.
.PP
In restricted mode, options are limited to those with names and values
known to be safe; some options taking booleans, integers or fixed
names are allowed, those taking general strings are not.

.SH EXAMPLES
Examples all equivalently converting `test.eps' to `test.pdf':
.nf
epstopdf test.eps
cat test.eps | epstopdf --filter >test.pdf
cat test.eps | epstopdf -f -o=test.pdf
.fi
.PP
Example for using HiResBoundingBox instead of BoundingBox:
.nf
epstopdf --hires test.eps
.fi
.PP
Example for producing \fBepstopdf\fP's attempt at corrected PostScript:
.nf
$program --nogs test.ps >testcorr.ps
.fi
.PP
In all cases, you can add \fB--debug\fP (\fB-d\fP) to see more about
what \fBepstopdf\fP is doing.
.SH BUGS
The case of "%%BoundingBox: (atend)" when input is not seekable (e.g.,
from a pipe) is not supported.
.PP
Report bugs in the program or this man page to tex-k@tug.org.  When
reporting bugs, please include an input file and the command line
options specified, so the problem can be reproduced.
.SH SEE ALSO
\fBgs\fP(1),
\fBpdfcrop\fP(1).
.PP
The epstopdf LaTeX package, part of the oberdiek bundle, which automates
running this script on the fly under TeX: http://ctan.org/pkg/epstopdf-pkg.
.SH AUTHOR
Originally written by Sebastian Rahtz, for Elsevier Science, with
subsequent contributions from Thomas Esser, Gerben Wierda, Heiko
Oberdiek, and many others.  Currently maintained by Karl Berry.
.PP
Man page originally written by Jim Van Zandt.
.PP
epstopdf home page: http://tug.org/epstopdf.
.PP
You may freely use, modify and/or distribute this file.

